Dynamics and Formation of the Near-Resonant K2-24 System: Insights from Transit-Timing Variations and Radial Velocities

While planets between the size of Uranus and Saturn are absent within the Solar System, the star K2-24 hosts two such planets, K2-24b and c, with radii equal to $5.4~R_E$ and $7.5~R_E$, respectively. The two planets have orbital periods of 20.9 days and 42.4 days, residing only 1% outside the nominal 2:1 mean-motion resonance. In this work, we present results from a coordinated observing campaign to measure planet masses and eccentricities that combines radial velocity (RV) measurements from Keck/HIRES and transit-timing measurements from K2 and Spitzer. K2-24b and c have low, but non-zero, eccentricities of $e_1 \sim e_2 \sim 0.08$. The low observed eccentricities provide clues regarding the formation and dynamical evolution of K2-24b and K2-24c, suggesting that they could be the result of stochastic gravitational interactions with a turbulent protoplanetary disk, among other mechanisms. K2-24b and c are $19\pm2~M_E$ and $15\pm2~M_E$, respectively; K2-24c is 20% less massive than K2-24b, despite being 40% larger. Their large sizes and low masses imply large envelope fractions, which we estimate at $26^{+3}_{-3}\%$ and $52^{+5}_{-3}\%$. In particular, K2-24c's large envelope presents an intriguing challenge to the standard model of core nucleated accretion that predicts the onset of runaway accretion when $f_{env} \approx 50\%$.

==> tab_rv.tex <==
2364.819580 & 0.85 & 1.68 & 0.132 \\
2364.825101 & 1.72 & 1.52 & 0.130 \\
2364.830703 & 9.99 & 1.59 & 0.132 \\
2366.827579 & -3.90 & 1.62 & 0.128 \\
2367.852646 & 5.50 & 1.65 & 0.130 \\
2373.888150 & -3.77 & 1.78 & 0.094 \\
2374.852412 & -5.65 & 1.97 & 0.113 \\
2376.863820 & -6.09 & 1.79 & 0.131 \\
2377.866073 & -2.40 & 1.76 & 0.131 \\
2378.834011 & -1.33 & 1.60 & 0.131 \\
2380.930797 & 8.23 & 1.93 & 0.128 \\
2382.886140 & 3.73 & 1.85 & 0.126 \\
2383.823529 & -0.97 & 1.89 & 0.130 \\
2384.799943 & -4.41 & 1.67 & 0.128 \\
2384.828991 & -1.39 & 1.65 & 0.131 \\
2384.839720 & -7.57 & 1.76 & 0.127 \\
2388.955960 & -4.60 & 1.92 & 0.119 \\
2395.857258 & -3.80 & 1.74 & 0.129 \\
2402.898756 & 4.81 & 1.78 & 0.124 \\
2403.771319 & 4.17 & 1.69 & 0.130 \\
2411.755697 & -8.79 & 1.58 & 0.129 \\
2412.794200 & -4.86 & 1.57 & 0.129 \\
2420.803019 & -3.13 & 1.76 & 0.128 \\
2421.822804 & -3.99 & 1.73 & 0.124 \\
2422.742125 & -1.46 & 1.80 & 0.121 \\
2429.761751 & -14.14 & 2.02 & 0.130 \\
2429.810230 & -12.80 & 1.85 & 0.131 \\
2432.732316 & -12.60 & 1.66 & 0.125 \\
2432.807239 & -13.94 & 1.92 & 0.119 \\
2457.716902 & 0.65 & 1.64 & 0.125 \\
2457.754804 & -6.33 & 1.90 & 0.118 \\
2465.710740 & 3.38 & 1.58 & 0.127 \\
2582.168372 & -3.88 & 1.72 & 0.133 \\
2607.130008 & -1.96 & 1.74 & 0.135 \\
2722.950539 & 4.04 & 1.85 & 0.133 \\
2728.989014 & 2.09 & 1.95 & 0.133 \\
2749.919339 & 5.10 & 1.71 & 0.128 \\
2762.878386 & 5.77 & 1.89 & 0.110 \\
2767.878283 & 0.87 & 1.73 & 0.115 \\
2784.782876 & 2.45 & 1.72 & 0.123 \\
2785.829743 & 1.97 & 1.66 & 0.125 \\
2819.713570 & 4.90 & 1.61 & 0.134 \\
2820.710621 & -0.43 & 2.09 & 0.117 \\
2956.169520 & -3.47 & 1.82 & 0.134 \\
2957.134774 & -0.08 & 1.67 & 0.127 \\
2960.171395 & 1.36 & 2.02 & 0.132 \\
2996.061096 & -1.54 & 1.80 & 0.130 \\
3020.973246 & -7.70 & 1.69 & 0.133 \\
3022.056539 & -6.44 & 1.89 & 0.143 \\
3055.035798 & 7.20 & 1.73 & 0.139 \\
3075.008617 & 1.42 & 1.85 & 0.131 \\
3091.974893 & 13.40 & 1.85 & 0.126 \\
3099.888450 & 0.37 & 1.61 & 0.127 \\
3100.818379 & 4.41 & 1.68 & 0.129 \\
3100.818379 & 4.41 & 1.68 & 0.129 \\
3101.846797 & -0.17 & 1.70 & 0.129 \\
3131.815608 & 14.20 & 1.65 & 0.127 \\
3138.845712 & 1.47 & 1.64 & 0.124 \\
3155.769495 & 5.82 & 1.82 & 0.126 \\
3169.777349 & 4.03 & 1.85 & 0.119 \\
3185.715366 & 2.19 & 1.84 & 0.133 \\
3186.715161 & -2.79 & 1.64 & 0.127 \\
3195.707773 & 0.92 & 1.92 & 0.125 \\
3196.706777 & 3.12 & 1.78 & 0.123 \\

==> tab_transit-times-predict.tex <==
b & 0 & 2014-09-05 & 2072.7962 & 0.0007 \\
c & 0 & 2014-09-15 & 2082.6250 & 0.0006 \\
b & 1 & 2014-09-26 & 2093.6803 & 0.0006 \\
b & 2 & 2014-10-17 & 2114.5650 & 0.0005 \\
c & 1 & 2014-10-27 & 2124.9877 & 0.0006 \\
b & 3 & 2014-11-06 & 2135.4505 & 0.0007 \\
b & 4 & 2014-11-27 & 2156.3366 & 0.0008 \\
c & 2 & 2014-12-08 & 2167.3449 & 0.0010 \\
b & 5 & 2014-12-18 & 2177.2235 & 0.0009 \\
b & 6 & 2015-01-08 & 2198.1112 & 0.0010 \\
c & 3 & 2015-01-20 & 2209.6958 & 0.0014 \\
b & 7 & 2015-01-29 & 2218.9997 & 0.0011 \\
b & 8 & 2015-02-19 & 2239.8889 & 0.0012 \\
c & 4 & 2015-03-03 & 2252.0403 & 0.0017 \\
b & 9 & 2015-03-12 & 2260.7790 & 0.0012 \\
b & 10 & 2015-04-02 & 2281.6698 & 0.0013 \\
c & 5 & 2015-04-14 & 2294.3781 & 0.0018 \\
b & 11 & 2015-04-23 & 2302.5614 & 0.0013 \\
b & 12 & 2015-05-13 & 2323.4538 & 0.0013 \\
c & 6 & 2015-05-27 & 2336.7092 & 0.0018 \\
b & 13 & 2015-06-03 & 2344.3469 & 0.0012 \\
b & 14 & 2015-06-24 & 2365.2407 & 0.0012 \\
c & 7 & 2015-07-08 & 2379.0340 & 0.0018 \\
b & 15 & 2015-07-15 & 2386.1352 & 0.0012 \\
b & 16 & 2015-08-05 & 2407.0305 & 0.0011 \\
c & 8 & 2015-08-19 & 2421.3529 & 0.0019 \\
b & 17 & 2015-08-26 & 2427.9263 & 0.0011 \\
b & 18 & 2015-09-16 & 2448.8227 & 0.0010 \\
c & 9 & 2015-10-01 & 2463.6663 & 0.0019 \\
b & 19 & 2015-10-07 & 2469.7197 & 0.0010 \\
b & 20 & 2015-10-28 & 2490.6172 & 0.0009 \\
c & 10 & 2015-11-12 & 2505.9751 & 0.0019 \\
b & 21 & 2015-11-18 & 2511.5151 & 0.0009 \\
b & 22 & 2015-12-08 & 2532.4134 & 0.0009 \\
c & 11 & 2015-12-24 & 2548.2800 & 0.0019 \\
b & 23 & 2015-12-29 & 2553.3120 & 0.0009 \\
b & 24 & 2016-01-19 & 2574.2109 & 0.0009 \\
c & 12 & 2016-02-05 & 2590.5822 & 0.0018 \\
b & 25 & 2016-02-09 & 2595.1099 & 0.0009 \\
b & 26 & 2016-03-01 & 2616.0091 & 0.0009 \\
c & 13 & 2016-03-18 & 2632.8825 & 0.0017 \\
b & 27 & 2016-03-22 & 2636.9084 & 0.0009 \\
b & 28 & 2016-04-12 & 2657.8077 & 0.0009 \\
c & 14 & 2016-04-29 & 2675.1820 & 0.0017 \\
b & 29 & 2016-05-03 & 2678.7070 & 0.0009 \\
b & 30 & 2016-05-24 & 2699.6060 & 0.0009 \\
c & 15 & 2016-06-10 & 2717.4820 & 0.0020 \\
b & 31 & 2016-06-14 & 2720.5049 & 0.0010 \\
b & 32 & 2016-07-04 & 2741.4036 & 0.0012 \\
c & 16 & 2016-07-23 & 2759.7835 & 0.0027 \\
b & 33 & 2016-07-25 & 2762.3020 & 0.0014 \\
b & 34 & 2016-08-15 & 2783.1999 & 0.0016 \\
c & 17 & 2016-09-03 & 2802.0876 & 0.0038 \\
b & 35 & 2016-09-05 & 2804.0974 & 0.0018 \\
b & 36 & 2016-09-26 & 2824.9945 & 0.0021 \\
c & 18 & 2016-10-15 & 2844.3953 & 0.0054 \\
b & 37 & 2016-10-17 & 2845.8910 & 0.0026 \\
b & 38 & 2016-11-07 & 2866.7869 & 0.0030 \\
c & 19 & 2016-11-27 & 2886.7074 & 0.0073 \\
b & 39 & 2016-11-28 & 2887.6822 & 0.0035 \\
b & 40 & 2016-12-19 & 2908.5769 & 0.0040 \\
c & 20 & 2017-01-08 & 2929.0249 & 0.0096 \\
b & 41 & 2017-01-08 & 2929.4709 & 0.0046 \\
b & 42 & 2017-01-29 & 2950.3641 & 0.0052 \\
b & 43 & 2017-02-19 & 2971.2565 & 0.0059 \\
c & 21 & 2017-02-19 & 2971.3483 & 0.0119 \\
b & 44 & 2017-03-12 & 2992.1482 & 0.0065 \\
b & 45 & 2017-04-02 & 3013.0391 & 0.0072 \\
c & 22 & 2017-04-03 & 3013.6781 & 0.0144 \\
b & 46 & 2017-04-23 & 3033.9293 & 0.0079 \\
b & 47 & 2017-05-14 & 3054.8187 & 0.0087 \\
c & 23 & 2017-05-15 & 3056.0145 & 0.0172 \\
b & 48 & 2017-06-04 & 3075.7072 & 0.0095 \\
b & 49 & 2017-06-25 & 3096.5949 & 0.0104 \\
c & 24 & 2017-06-26 & 3098.3572 & 0.0203 \\
b & 50 & 2017-07-15 & 3117.4820 & 0.0112 \\
b & 51 & 2017-08-05 & 3138.3682 & 0.0121 \\
c & 25 & 2017-08-08 & 3140.7064 & 0.0234 \\
b & 52 & 2017-08-26 & 3159.2538 & 0.0129 \\
b & 53 & 2017-09-16 & 3180.1386 & 0.0137 \\
c & 26 & 2017-09-19 & 3183.0620 & 0.0267 \\
b & 54 & 2017-10-07 & 3201.0229 & 0.0145 \\
b & 55 & 2017-10-28 & 3221.9065 & 0.0153 \\
c & 27 & 2017-10-31 & 3225.4232 & 0.0299 \\
b & 56 & 2017-11-18 & 3242.7894 & 0.0161 \\
b & 57 & 2017-12-09 & 3263.6719 & 0.0169 \\
c & 28 & 2017-12-13 & 3267.7900 & 0.0328 \\
b & 58 & 2017-12-30 & 3284.5539 & 0.0177 \\
b & 59 & 2018-01-19 & 3305.4354 & 0.0184 \\
c & 29 & 2018-01-24 & 3310.1613 & 0.0357 \\
b & 60 & 2018-02-09 & 3326.3166 & 0.0191 \\
b & 61 & 2018-03-02 & 3347.1974 & 0.0199 \\
c & 30 & 2018-03-08 & 3352.5357 & 0.0383 \\
b & 62 & 2018-03-23 & 3368.0779 & 0.0206 \\
b & 63 & 2018-04-13 & 3388.9582 & 0.0213 \\
c & 31 & 2018-04-19 & 3394.9127 & 0.0408 \\
b & 64 & 2018-05-04 & 3409.8384 & 0.0219 \\
b & 65 & 2018-05-25 & 3430.7185 & 0.0226 \\
c & 32 & 2018-05-31 & 3437.2915 & 0.0429 \\
b & 66 & 2018-06-15 & 3451.5986 & 0.0231 \\
b & 67 & 2018-07-05 & 3472.4793 & 0.0238 \\
c & 33 & 2018-07-13 & 3479.6701 & 0.0448 \\
b & 68 & 2018-07-26 & 3493.3598 & 0.0244 \\
b & 69 & 2018-08-16 & 3514.2406 & 0.0248 \\
c & 34 & 2018-08-24 & 3522.0483 & 0.0461 \\
b & 70 & 2018-09-06 & 3535.1216 & 0.0252 \\
b & 71 & 2018-09-27 & 3556.0028 & 0.0256 \\
c & 35 & 2018-10-05 & 3564.4240 & 0.0471 \\
b & 72 & 2018-10-18 & 3576.8844 & 0.0259 \\
b & 73 & 2018-11-08 & 3597.7664 & 0.0261 \\
c & 36 & 2018-11-17 & 3606.7969 & 0.0481 \\
b & 74 & 2018-11-29 & 3618.6488 & 0.0261 \\
b & 75 & 2018-12-20 & 3639.5318 & 0.0263 \\
c & 37 & 2018-12-29 & 3649.1666 & 0.0485 \\
b & 76 & 2019-01-09 & 3660.4156 & 0.0265 \\
b & 77 & 2019-01-30 & 3681.3000 & 0.0267 \\
c & 38 & 2019-02-10 & 3691.5311 & 0.0487 \\
b & 78 & 2019-02-20 & 3702.1850 & 0.0269 \\
b & 79 & 2019-03-13 & 3723.0708 & 0.0269 \\
c & 39 & 2019-03-24 & 3733.8900 & 0.0483 \\
b & 80 & 2019-04-03 & 3743.9570 & 0.0268 \\
b & 81 & 2019-04-24 & 3764.8444 & 0.0268 \\
c & 40 & 2019-05-05 & 3776.2430 & 0.0479 \\
b & 82 & 2019-05-15 & 3785.7323 & 0.0268 \\
b & 83 & 2019-06-05 & 3806.6210 & 0.0266 \\
c & 41 & 2019-06-17 & 3818.5896 & 0.0469 \\
b & 84 & 2019-06-26 & 3827.5104 & 0.0265 \\
b & 85 & 2019-07-16 & 3848.4008 & 0.0264 \\
c & 42 & 2019-07-29 & 3860.9298 & 0.0458 \\
b & 86 & 2019-08-06 & 3869.2919 & 0.0262 \\
b & 87 & 2019-08-27 & 3890.1838 & 0.0259 \\
c & 43 & 2019-09-09 & 3903.2632 & 0.0447 \\
b & 88 & 2019-09-17 & 3911.0764 & 0.0257 \\
b & 89 & 2019-10-08 & 3931.9698 & 0.0255 \\
c & 44 & 2019-10-22 & 3945.5900 & 0.0436 \\
b & 90 & 2019-10-29 & 3952.8639 & 0.0252 \\
b & 91 & 2019-11-19 & 3973.7587 & 0.0249 \\
c & 45 & 2019-12-03 & 3987.9107 & 0.0426 \\
b & 92 & 2019-12-10 & 3994.6541 & 0.0246 \\
b & 93 & 2019-12-31 & 4015.5502 & 0.0243 \\
c & 46 & 2020-01-14 & 4030.2258 & 0.0416 \\
b & 94 & 2020-01-20 & 4036.4468 & 0.0241 \\
b & 95 & 2020-02-10 & 4057.3440 & 0.0239 \\
c & 47 & 2020-02-26 & 4072.5358 & 0.0407 \\
b & 96 & 2020-03-02 & 4078.2416 & 0.0236 \\
b & 97 & 2020-03-23 & 4099.1397 & 0.0234 \\
c & 48 & 2020-04-08 & 4114.8416 & 0.0402 \\
b & 98 & 2020-04-13 & 4120.0382 & 0.0233 \\
b & 99 & 2020-05-04 & 4140.9369 & 0.0231 \\
c & 49 & 2020-05-20 & 4157.1445 & 0.0400 \\
b & 100 & 2020-05-25 & 4161.8358 & 0.0229 \\
b & 101 & 2020-06-15 & 4182.7350 & 0.0229 \\
c & 50 & 2020-07-01 & 4199.4453 & 0.0398 \\
b & 102 & 2020-07-06 & 4203.6343 & 0.0229 \\
b & 103 & 2020-07-27 & 4224.5337 & 0.0229 \\
c & 51 & 2020-08-13 & 4241.7451 & 0.0404 \\
b & 104 & 2020-08-16 & 4245.4329 & 0.0231 \\
b & 105 & 2020-09-06 & 4266.3320 & 0.0233 \\
c & 52 & 2020-09-24 & 4284.0448 & 0.0413 \\
b & 106 & 2020-09-27 & 4287.2309 & 0.0236 \\
b & 107 & 2020-10-18 & 4308.1298 & 0.0239 \\
c & 53 & 2020-11-05 & 4326.3459 & 0.0426 \\
b & 108 & 2020-11-08 & 4329.0283 & 0.0241 \\
b & 109 & 2020-11-29 & 4349.9265 & 0.0244 \\
c & 54 & 2020-12-18 & 4368.6491 & 0.0442 \\
b & 110 & 2020-12-20 & 4370.8243 & 0.0248 \\
b & 111 & 2021-01-10 & 4391.7217 & 0.0253 \\
c & 55 & 2021-01-29 & 4410.9554 & 0.0461 \\
b & 112 & 2021-01-31 & 4412.6186 & 0.0257 \\
b & 113 & 2021-02-21 & 4433.5150 & 0.0262 \\
c & 56 & 2021-03-12 & 4453.2662 & 0.0485 \\
b & 114 & 2021-03-13 & 4454.4107 & 0.0267 \\
b & 115 & 2021-04-03 & 4475.3057 & 0.0274 \\
c & 57 & 2021-04-24 & 4495.5822 & 0.0513 \\
b & 116 & 2021-04-24 & 4496.2001 & 0.0280 \\
b & 117 & 2021-05-15 & 4517.0938 & 0.0288 \\
c & 58 & 2021-06-05 & 4537.9034 & 0.0543 \\
b & 118 & 2021-06-05 & 4537.9866 & 0.0296 \\
b & 119 & 2021-06-26 & 4558.8788 & 0.0305 \\
b & 120 & 2021-07-17 & 4579.7703 & 0.0313 \\
c & 59 & 2021-07-17 & 4580.2308 & 0.0577 \\
b & 121 & 2021-08-07 & 4600.6609 & 0.0323 \\
b & 122 & 2021-08-28 & 4621.5508 & 0.0333 \\
c & 60 & 2021-08-29 & 4622.5650 & 0.0616 \\
b & 123 & 2021-09-17 & 4642.4398 & 0.0343 \\
b & 124 & 2021-10-08 & 4663.3280 & 0.0352 \\
c & 61 & 2021-10-10 & 4664.9056 & 0.0654 \\
b & 125 & 2021-10-29 & 4684.2156 & 0.0362 \\
b & 126 & 2021-11-19 & 4705.1023 & 0.0372 \\
c & 62 & 2021-11-21 & 4707.2529 & 0.0691 \\
b & 127 & 2021-12-10 & 4725.9883 & 0.0382 \\
b & 128 & 2021-12-31 & 4746.8736 & 0.0392 \\
c & 63 & 2022-01-03 & 4749.6065 & 0.0730 \\
b & 129 & 2022-01-21 & 4767.7582 & 0.0403 \\
b & 130 & 2022-02-11 & 4788.6422 & 0.0413 \\
c & 64 & 2022-02-14 & 4791.9662 & 0.0769 \\
b & 131 & 2022-03-04 & 4809.5257 & 0.0423 \\
b & 132 & 2022-03-24 & 4830.4086 & 0.0432 \\
c & 65 & 2022-03-28 & 4834.3313 & 0.0805 \\
b & 133 & 2022-04-14 & 4851.2908 & 0.0441 \\
b & 134 & 2022-05-05 & 4872.1726 & 0.0451 \\
c & 66 & 2022-05-10 & 4876.7012 & 0.0840 \\
b & 135 & 2022-05-26 & 4893.0538 & 0.0460 \\
b & 136 & 2022-06-16 & 4913.9349 & 0.0469 \\
c & 67 & 2022-06-21 & 4919.0746 & 0.0872 \\
b & 137 & 2022-07-07 & 4934.8159 & 0.0477 \\
b & 138 & 2022-07-28 & 4955.6964 & 0.0484 \\
c & 68 & 2022-08-02 & 4961.4511 & 0.0902 \\
b & 139 & 2022-08-18 & 4976.5767 & 0.0491 \\
b & 140 & 2022-09-07 & 4997.4569 & 0.0497 \\
c & 69 & 2022-09-14 & 5003.8291 & 0.0925 \\
b & 141 & 2022-09-28 & 5018.3372 & 0.0503 \\
b & 142 & 2022-10-19 & 5039.2175 & 0.0508 \\
c & 70 & 2022-10-26 & 5046.2073 & 0.0942 \\
b & 143 & 2022-11-09 & 5060.0979 & 0.0513 \\
b & 144 & 2022-11-30 & 5080.9784 & 0.0517 \\
c & 71 & 2022-12-08 & 5088.5854 & 0.0962 \\
b & 145 & 2022-12-21 & 5101.8590 & 0.0521 \\
b & 146 & 2023-01-11 & 5122.7400 & 0.0524 \\
c & 72 & 2023-01-19 & 5130.9626 & 0.0975 \\
b & 147 & 2023-02-01 & 5143.6214 & 0.0527 \\
b & 148 & 2023-02-22 & 5164.5031 & 0.0531 \\
c & 73 & 2023-03-02 & 5173.3368 & 0.0982 \\
b & 149 & 2023-03-14 & 5185.3855 & 0.0532 \\
b & 150 & 2023-04-04 & 5206.2683 & 0.0532 \\
c & 74 & 2023-04-14 & 5215.7077 & 0.0977 \\
b & 151 & 2023-04-25 & 5227.1517 & 0.0533 \\
b & 152 & 2023-05-16 & 5248.0355 & 0.0532 \\
c & 75 & 2023-05-26 & 5258.0737 & 0.0970 \\
b & 153 & 2023-06-06 & 5268.9200 & 0.0532 \\
b & 154 & 2023-06-27 & 5289.8053 & 0.0531 \\
c & 76 & 2023-07-07 & 5300.4343 & 0.0964 \\
b & 155 & 2023-07-18 & 5310.6912 & 0.0528 \\
b & 156 & 2023-08-08 & 5331.5778 & 0.0527 \\
c & 77 & 2023-08-19 & 5342.7897 & 0.0952 \\
b & 157 & 2023-08-28 & 5352.4652 & 0.0525 \\
b & 158 & 2023-09-18 & 5373.3534 & 0.0522 \\
c & 78 & 2023-09-30 & 5385.1384 & 0.0937 \\
b & 159 & 2023-10-09 & 5394.2425 & 0.0519 \\
b & 160 & 2023-10-30 & 5415.1323 & 0.0516 \\
c & 79 & 2023-11-11 & 5427.4802 & 0.0919 \\
b & 161 & 2023-11-20 & 5436.0229 & 0.0513 \\
b & 162 & 2023-12-11 & 5456.9142 & 0.0509 \\
c & 80 & 2023-12-24 & 5469.8152 & 0.0896 \\
b & 163 & 2024-01-01 & 5477.8062 & 0.0504 \\
b & 164 & 2024-01-22 & 5498.6991 & 0.0500 \\
c & 81 & 2024-02-04 & 5512.1441 & 0.0872 \\
b & 165 & 2024-02-12 & 5519.5928 & 0.0496 \\
b & 166 & 2024-03-03 & 5540.4872 & 0.0493 \\
c & 82 & 2024-03-17 & 5554.4670 & 0.0852 \\
b & 167 & 2024-03-24 & 5561.3823 & 0.0489 \\
b & 168 & 2024-04-14 & 5582.2780 & 0.0485 \\
c & 83 & 2024-04-29 & 5596.7841 & 0.0837 \\
b & 169 & 2024-05-05 & 5603.1743 & 0.0481 \\
b & 170 & 2024-05-26 & 5624.0712 & 0.0478 \\
c & 84 & 2024-06-10 & 5639.0958 & 0.0825 \\
b & 171 & 2024-06-16 & 5644.9685 & 0.0474 \\
b & 172 & 2024-07-07 & 5665.8663 & 0.0472 \\
c & 85 & 2024-07-22 & 5681.4032 & 0.0815 \\
b & 173 & 2024-07-28 & 5686.7646 & 0.0469 \\
b & 174 & 2024-08-18 & 5707.6632 & 0.0468 \\
c & 86 & 2024-09-03 & 5723.7066 & 0.0808 \\
b & 175 & 2024-09-08 & 5728.5620 & 0.0466 \\
b & 176 & 2024-09-28 & 5749.4610 & 0.0465 \\
c & 87 & 2024-10-15 & 5766.0079 & 0.0805 \\
b & 177 & 2024-10-19 & 5770.3602 & 0.0465 \\
b & 178 & 2024-11-09 & 5791.2596 & 0.0465 \\
c & 88 & 2024-11-26 & 5808.3083 & 0.0806 \\
b & 179 & 2024-11-30 & 5812.1587 & 0.0465 \\
b & 180 & 2024-12-21 & 5833.0579 & 0.0466 \\
c & 89 & 2025-01-08 & 5850.6084 & 0.0810 \\
b & 181 & 2025-01-11 & 5853.9570 & 0.0468 \\
b & 182 & 2025-02-01 & 5874.8560 & 0.0471 \\
c & 90 & 2025-02-19 & 5892.9089 & 0.0825 \\
b & 183 & 2025-02-22 & 5895.7547 & 0.0474 \\
b & 184 & 2025-03-15 & 5916.6529 & 0.0477 \\
c & 91 & 2025-04-02 & 5935.2113 & 0.0843 \\
b & 185 & 2025-04-05 & 5937.5511 & 0.0481 \\
b & 186 & 2025-04-25 & 5958.4487 & 0.0486 \\
c & 92 & 2025-05-15 & 5977.5169 & 0.0864 \\
b & 187 & 2025-05-16 & 5979.3457 & 0.0492 \\
b & 188 & 2025-06-06 & 6000.2423 & 0.0498 \\
c & 93 & 2025-06-26 & 6019.8257 & 0.0894 \\
b & 189 & 2025-06-27 & 6021.1386 & 0.0504 \\
b & 190 & 2025-07-18 & 6042.0341 & 0.0510 \\
c & 94 & 2025-08-07 & 6062.1392 & 0.0927 \\
b & 191 & 2025-08-08 & 6062.9290 & 0.0518 \\
b & 192 & 2025-08-29 & 6083.8233 & 0.0526 \\
c & 95 & 2025-09-18 & 6104.4585 & 0.0966 \\
b & 193 & 2025-09-19 & 6104.7165 & 0.0535 \\
b & 194 & 2025-10-10 & 6125.6091 & 0.0546 \\
b & 195 & 2025-10-31 & 6146.5011 & 0.0556 \\
c & 96 & 2025-10-31 & 6146.7839 & 0.1006 \\
b & 196 & 2025-11-20 & 6167.3924 & 0.0567 \\
b & 197 & 2025-12-11 & 6188.2829 & 0.0578 \\
c & 97 & 2025-12-12 & 6189.1158 & 0.1048 \\
